Monitoring Constraints in Business Processes Using Object-Centric Constraint Graphs

Constraint monitoring aims to monitor the violation of constraints in business processes, e.g., an invoice should be cleared within 48 hours after the corresponding goods receipt, by analyzing event data. Existing techniques for constraint monitoring assume that a single case notion exists in a business process, e.g., a patient in a healthcare process, and each event is associated with the case notion. However, in reality, business processes are object-centric, i.e., multiple case notions (objects) exist, and an event may be associated with multiple objects. For instance, an Order-To-Cash (O2C) process involves order, item, delivery, etc., and they interact when executing an event, e.g., packing multiple items together for a delivery. The existing techniques produce misleading insights when applied to such object-centric business processes. In this work, we propose an approach to monitoring constraints in object-centric business processes. To this end, we introduce Object-Centric Constraint Graphs (OCCGs) to represent constraints that consider the interaction of objects. Next, we evaluate the constraints represented by OCCGs by analyzing Object-Centric Event Logs (OCELs) that store the interaction of different objects in events. We have implemented a web application to support the proposed approach and conducted two case studies using a real-life SAP ERP system.

==> Sections/6-Monitoring.tex <==
\section{Monitoring: An Approach based on Pattern Graphs}\label{sec:approach}
This section introduces a pattern monitoring engine to evaluate the existence of problem patterns, represented as pattern graphs, by analyzing OCELs.

\begin{definition}[Pattern Monitoring Engine]
A pattern monitoring engine $\mi{monitor} \in \univ{L} \times \univ{cg} \rightarrow \{\mi{true},\mi{false}\}$ is a function that maps an object-centric event log and a pattern graph to a Boolean value.
For any $L \in \univ{L}$ and $cg \in \univ{cg}$,  $\mi{monitor}(L,cg)=\mi{true}$ if $cg$ $\mi{exists}$ in $\mi{L}$, and $\mi{false}$, otherwise.
\end{definition}

As shown in \autoref{fig:approach}, we implement the pattern monitoring engine by 1) computing ordering relations, object involvements, and diagnostics of an OCEL and 2) evaluating the existence of the pattern graphs based on them.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/approach.png}
    \caption{An overview of the monitoring approach.}
    \label{fig:approach}
\end{figure}

The derivation of ordering relations and object involvements is deterministic according to \autoref{def:or} and \autoref{def:oi}, respectively.
However, the computation of diagnostics is non-trivial. 
In this work, we use the approach proposed in~\cite{https://doi.org/10.48550/arxiv.2204.10662} to compute diagnostics including \emph{flow time}, \emph{synchronization time}, \emph{pooling time}, and \emph{lagging time} along with more traditional metrics such as \emph{sojourn time}, \emph{waiting time}, \emph{service time}.

The approach first discovers an OCPN from an OCEL by following the general approach, presented in \cite{DBLP:journals/fuin/AalstB20}.
The proposed approach leverages existing process discovery techniques for flattened event data.
More in detail, it first flattens an OCEL to flattened event logs, each of which corresponds to an object type.
Next, it discovers an accepting Petri net from the flattened event log using any conventional discovery technique.
Afterward, it merges the accepting Petri nets into a Petri net and assigns object types to the places.
Finally, it identifies variable arcs, completing an object-centric Petri net.

Next, the approach couples events in an OCEL to an OCPN by ``playing the token game'' and computes performance measures such as \emph{flow time}, \emph{synchronization time}, \emph{pooling time}, and \emph{lagging time} along with more traditional metrics such as \emph{sojourn time}, \emph{waiting time}, \emph{service time}.

Finally, Given a pattern graph, an accepting object-centric Petri net, and an enhancement, the evaluation is deterministic according to \autoref{def:semantics}.

==> Sections/X-Approach.tex <==
\section{An Approach to Object-Centric Performance Analysis}\label{sec:formal-derivation}


The process discovery follows the generic approach proposed in \cite{DBLP:journals/fuin/AalstB20}.
In the remainder of this section, we formally define the following steps and explain concrete instantiations.
% and provide an instantiation of the step.

\subsection{Filtering Events of Process Instances}
% Based on a provided analysis view, we filter events in process instances so that relevant event data are used to measure performance metrics.
Based on a provided analysis view, we filter an OCEL so that relevant events are used to measure performance measures.


\begin{definition}[Event Filter]
Let $L{=}(E,\prec_{E})$ be an object-centric event log and $\mi{AN}{=}(\mi{ON},M_{\mi{init}},M_{\mi{final}})$ an accepting object-centric Petri net with $ON{=}(N,\\ \mathit{pt},F_{\mathit{var}})$ and $N{=}(P,T,F,l)$. 
% Let $\mathit{ON}{=}(N,\mathit{pt},F_{\mathit{var}})$ be an object-centric Petri net with $N{=}(P,T,F,l)$ and 
Let $av{=}(T_{av},OT_{av}) \in AV_{AN}$ be a consistent analysis view.
$filt(L,av){=}(E',\prec_{E'})$ where $E'{=}\{ e \in E \mid \exists_{ot \in OT_{av}} \: \pi_{omap}(e)(ot) \neq \perp \land \pi_{act}(e) \in \{ l(t) \mid t \in T_{av} \} \}$
such that $\forall_{e_1,e_2 \in E'} \ e_1 \prec_{E'} e_2 \ \Rightarrow \ \pim{ct}(e_1) \leq \pim{ct}(e_2)$.
\end{definition}

% \begin{definition}[Event Filter]
% Let $L=(E,\prec_{E})$ be an object-centric event log.
% Let $\mathit{ON}{=}(N,\mathit{pt},F_{\mathit{var}})$ be an object-centric Petri net with $N{=}(P,T,F,l)$ and $av=(T_{av},OT_{av})$ a consistent analysis view of $ON$.
% Let $pi=(V,K)$ be a process instance.
% $filt_{av}(pi)=(V',K')$ where $E'=\{ e \in V \mid \exists_{ot \in OT_{av}} \: \pi_{omap}(e)(ot) \neq \perp \land \pi_{act}(e) \in \{ l(t) \mid t \in T_{av} \} \}$.
% \end{definition}

For instance, given the event data in \autoref{fig:motivation}(a), $L_1$, and $av'{=}(\{Item,Order\},\{t1,\\t2\})$ where $l(t1){=}\textit{place order}$ and $l(t2){=}\textit{collect payment}$, $filt(L_1,av'){=}(E,\prec_{E})$ such that $\{e1,e4,e7\} \subseteq E$.

\subsection{Projecting Object-Centric Petri Nets}
Next, we project OCPNs on a provided analysis view such that the projected net describes process behaviors defined over the view.
% A model projector is a function that projects OCPNs given views.

% \begin{definition}[Object Projection]\label{def:object-projection}
% Let $\mathit{ON}{=}(N,\mathit{pt},F_{\mathit{var}})$ be an object-centric Petri net.
% Let $OT' \subseteq type(ON)$ be a set of object types.
% An object projection $proj_{obj}(ON,OT')=(N',\mathit{pt}',F'_{\mathit{var}})$ with $N'{=}(P',T',F',l')$, where
% \begin{itemize}
%     % \item $\overline{P}=\{p \in P | pt(p) \in OT'\}$
%     \item $P' \subseteq \{p \in P | pt(p) \in OT'\}$
%     \item $T'=\{t \in T | \exists{ot \in tpl(t)} \: ot \in OT' \in \}$
%     \item $F'=\{(s,t) \in F | (s,t) \in (P'\times T') \cup (T' \times P') \}$
%     \item $l' \in T' \nrightarrow \univ{act}$ such that, for any $t \in T'$, $l'(t)=l(t)$
%     \item $pt' \in P' \to \univ{oi}$ such that, for any $p \in P'$, $pt'(p)=pt(p)$
%     \item $F'_{\mathit{var}}=\{f \in F_{var} | f \in F'\}$.
% \end{itemize}
% \end{definition}

\begin{definition}[Model Projection]\label{def:object-projection}
% Let $\mathit{ON}{=}(N,\mathit{pt},F_{\mathit{var}})$ be an object-centric Petri net with $N{=}(P,T,F,l)$. 
Let $\mi{AN}{=}(\mi{ON},M_{\mi{init}},M_{\mi{final}})$ be an accepting object-centric Petri net. 
Let $av \in AV_{AN}$ be a consistent analysis view. 
% A projection $proj_{ON} \in (\widehat{AN}_{ON} \times \widehat{AV}_{ON}) \rightarrow \widehat{AN}_{P(ON)}$ assigns accepting object-centric Petri nets of $ON$ to accepting object-centric Petri nets of $PN_{av}$.
A projection $proj_{AN} \in AV_{AN} \rightarrow PN_{AN}$ assigns analysis views of $AN$ to projected nets of $AN$.
\end{definition}

We instantiate the model projection function in two steps.
First, we project an OCPN on object types by removing places of non-selected object types and transitions only having such places as input/output places.
% Projecting OCPN on object types is rather trivial. We can remove places of non-selected object types and transitions only having such places as input/output places.
Assume we project the OCPN in \autoref{fig:projection-example}(a) on $av_{2}$ introduced in \autoref{sec:performance-metric}.
As depicted in \autoref{fig:reduction-example}(a), we remove order places (i.e., \textit{p1}, \textit{p3}, \textit{p6}, \textit{p8}, and \textit{p12}) and transitions only related to such places (i.e., \textit{t2}, \textit{t3}, and \textit{t6}) from the original OCPN.

\vspace{-0.5cm}
\begin{figure}[!htb]
    \centering
    \includegraphics[width=1\linewidth]{Figures/reduction-example.png}
    \caption{(a) projecting on object types, (b) hiding non-selected transitions, and (c) reducing nets}
    \label{fig:reduction-example}
\end{figure}
\vspace{-0.5cm}

% However, there exist multiple possible ways to project an OCPN on transitions. 
Next, we further project the OCPN on the selected transitions by hiding (making invisible) non-selected transitions and reducing the OCPN.
% Projecting an OCPN on transitions is non-trivial.
% In this work, we project an OCPN on selected transitions first by hiding (making invisible) non-selected transitions of the net and then reducing the net.

\begin{definition}[Hiding]\label{def:object-projection}
% Let $\mathit{ON}{=}(N,\mathit{pt},F_{\mathit{var}})$ be an object-centric Petri net with $N{=}(P,T,F,l)$. 
Let $\mi{AN}{=}(\mi{ON},M_{\mi{init}},M_{\mi{final}})$ be an accepting object-centric Petri net with $ON{=}(N,\mathit{pt},F_{\mathit{var}})$ and $N{=}(P,T,F,l)$. 
Let $av \in AV_{AN}$ be a consistent analysis view. 
% A hiding function $hide$ makes non-selected transitions invisible, i.e., $hide(ON,av){=}(N,\mathit{pt},F_{\mathit{var}}))$ with $N{=}(P,T,F,l_{av})$ such that
$H(AN,av){=}(\mi{ON},M_{\mi{init}},M_{\mi{final}})$ with  $\mi{ON}{=}(N,\mathit{pt},F_{\mathit{var}})$ and $N{=}(P,T,F,l')$ such that
\vspace{-0.25cm}
\[ 
l'(t) = \left\{
\begin{array}{ll}
      l(t) & \text{if } t \in T_{av} \\
      \tau & \text{if } t \notin T_{av}.
\end{array} 
\right. 
\]
\end{definition}
\vspace{-0.25cm}

As shown in \autoref{fig:reduction-example}(b), we make non-selected transitions (i.e., \textit{t1}, \textit{t4}, \textit{t5}, and \textit{t7}) invisible such that only the behavior of the selected transitions is described.

Next, we reduce the resulting net using Petri net reduction rules~\cite{24143}.
This makes the net as compact as possible while maintaining the behavior of the net.
For details of the Petri net reduction rules, we refer readers to~\cite{24143}.

In \autoref{fig:reduction-example}(c), we reduce \textit{p2}, \textit{t1}, and \textit{p4} to \textit{p4} by applying FSP rule. Next, we reduce \textit{t4} and \textit{t5} to \textit{t5} by applying FPT rule, after which \textit{p4}, \textit{t5}, and \textit{p5} is reduced to \textit{p5}. Finally, we reduce \textit{p5}, \textit{t7}, and \textit{p7} to \textit{p7}, resulting in the projected net in \autoref{fig:projection-example}(c).

\subsection{Measuring Performance Metrics}
Given the projected net and filtered OCEL, a performance measurement function measures a performance metric.
The range of the function is generalized as multi-sets of rational numbers, e.g., multi-set of throughput times by process instances.
% To this end, we 1) compute process instances, 2) replay the events in the process instances, and 3) measure the performance metric.
% A performance measurement function measures a performance metric given an OCEL and a projected net.
% We generalize the range of the function as multi-sets of rational numbers, e.g., multi-sets of throughput times by different process instances.
% Note that a multi-set may contain a single element, e.g., the absolute frequency of all process instances.
% Possibly, performance measures are not available for some domains (example required).

\begin{definition}[Performance Measurement]\label{def:performance-measurement}
Let $\mi{AN}{=}(\mi{ON},M_{\mi{init}},M_{\mi{final}})$ be an accepting object-centric Petri net.
% Let $\mathit{ON}{=}(N,\mathit{pt},F_{\mathit{var}})$ be an object-centric Petri net, where $N{=}(P,T,F,l)$.
% Let $L{=}(E,\prec_{E})$ be an object-centric event log.
$measure_{AN} \in \univ{EL} \times PN_{AN} \rightarrow \bag(\mathit{R}) \cup \{ \perp \}$ maps a filtered OCEL and a projected net to a multi-set of performance measures.
\end{definition}

% Computing performance measures using non-fitting OCELs and OCPNs is a remaining challenge in object-centric process mining. 
\autoref{tab:formal-derivation} formally describes the measurement functions to derive the metrics introduced in \autoref{tab:performance-metrics}.
In this work, we instantiate them, assuming that a given OCEL is completely replayable on the projected net \cite{DBLP:conf/icpm/AdamsA21}. 
Besides, the instantiation uses an enabler function $en_{AN}$ of an accepting object-centric Petri net $AN$ to relate the semantics of $AN$ to event data.
$en_{AN} \in (\univ{event} \times \univ{ot}) \nrightarrow \univ{event}$ relates an event and an object type to the preceding event that 1) is associated with the object type and 2) enabled the event (i.e., the transition related to the activity of the event).
% Note that, to simplify matters, we denote the enablement of an event as the enablement of the transition labeled with the activity of the event.
Given $AN'$ depicted in \autoref{fig:projection-example}(a) and $e \in \univ{event}$ such that $\pi_{act}(e)=\textit{start route}$,
$\pi_{act}(en_{AN'}(e,Item)){=}\textit{pick item}$, i.e., the event of \textit{pick item} is the preceding event of $e$.
% In this section, we deliberately abstract from the definition of $en_{AN}$. 
In \autoref{sec:evaluation}, we introduce an implementation based on event object graphs.
% , i.e., $en_{AN'}(e)=e'' \in E_{en}$ such that  $\forall_{E_{en}} \: \pi_{time}(e'') \ge \pi_{time}(e')$ where $E_{en}{=}\{ en_{AN'}(e,ot) | ot \in dom(pt) \} \setminus \perp$.

% Given object-centric event log $L$, object-centric Petri net $ON$, and sub-process $S$, we instantiate a measurement function $measure_{inst}$ as follows: 
% \begin{enumerate}
%     \item 
%     % In the instantiation, we only consider OCELs perfectly fitting to OCPNs for measuring performance metrics.
%     % To this end, we compute the fitness of a given OCEL, $L_{S}$, to a given OCPN, $ON_{S}$, based on the technique suggested in [].
%     % In case that the OCEL is not perfectly fitting, no valid measurement values are available, i.e., $measure_{inst}(L_S,ON_S)=\perp$.
%     \item According to \autoref{def:correlated-event-graph}, we derive process instances $PI_{filt(L,S)}$.
%     \item 
%     Based on process instances $PI_{filt(L,S)}$, we compute performance measures.
%     \autoref{tab:formal-derivation} describes the formal derivation of performance metrics.
% \end{enumerate}

% % We define a subprocess as a set of transitions whose sequence valid as a behavioral sequence in a process model, i.e., a subprocess of $\mathit{ON}{=}(N,\mathit{pt},F_{\mathit{var}})$ with $N{=}(P,T,F,l)$ is defined as $T' \subseteq T$ such that $\exists_{\sigma \in {T'}^*} \: \sigma \in \Phi(ON)$.

\begin{table}[h]
\centering
\caption{
% Let $\mathit{ON}{=}(N,\mathit{pt},F_{\mathit{var}})$ be an object-centric Petri net, where $N{=}(P,T,F,l)$.
% Let $S$ is a subprocess of $ON$.
% We assume that $L_{S}$ is perfectly fitting $ON_{S}$.
% $ctx_{OT'}(e)=\bigcup_{ot \in OT'} ctx(e,ot)$
% Formal derivation of performance metrics using $L_{av}$ and $PN_{av}$ such that $fit(L_{av},PN_{av})=1$. 
Let $AN$ be an accepting object-centric Petri net, $L$ an object-centric event log, and $av \in AV_{AN}$ an analysis view.
$PN'{=}proj_{AN}(av)$ is a projected net and $L'{=}filt(L,av)$ is a filtered object-centric event log replayable on $PN'$.
Given $pi{=}(E,K) \in PI_{L'}$, $first(pi)$/$last(pi)$ denote first/last events in $pi$.
% $last(pi) = \{e \in E \mid \forall_{e' \in E} \: e'\prec_{E} e \}$ and $first(pi) = \{e \in E \mid \forall_{e' \in E} \: e\prec_{E} e' \}$.
% Enablement function $en \in E \rightarrow \pow(E)$ maps an event to a set of events enabling the event.
Given $e \in \univ{event}$, $en_{AN}(e)$ denotes the latest enabling event of $e$ for any object types.
}
\smallskip
\sisetup{table-format = 3.2}
\setlength\tabcolsep{1.5pt}
\begin{tabularx}{\linewidth}{>{\hsize=0.3\hsize}X
                              >{\hsize=0.7\hsize}Y}  
\toprule 
\textbf{Performance Metric}  & \textbf{Formal Derivation} \\ 
\midrule
\textbf{Temporal Metric} & \\
\rowcolor[gray]{.9} 
Waiting time& $wait(L',PN'){=}[\pi_{st}(e){-}\pi_{ct}(e') \mid pi \in PI_{L'} \land e{=}first(pi) \land e'{=}en_{PN'}(e) ]$ \\ 
Service time     & $service(L',PN'){=}[\pi_{ct}(e){-}\pi_{st}(e') \mid pi \in PI_{L'} \land  e{=}last(pi) \land e'{=}first(pi) ]$ \\
\rowcolor[gray]{.9} 
% Sojourn time & $[\pi_{ct}(e){-}\pi_{ct}(e') \mid pi \in PI_{filt(L',S)} \land e{=}last(pi) \land e'{=}last(ctx(first(pi)))]$ \\
Sojourn time & $sojourn(L',PN'){=}[\pi_{ct}(e){-}\pi_{ct}(e') \mid pi \in PI_{L'} \land  e{=}last(pi) \land e'{=}en_{PN'}(first(pi))]$ \\
% Syncronization time& $[|\pi_{ct}(e''){-}\pi_{ct}(e')| \mid pi \in PI_{filt(L',S)} \land e{=}first(pi) \land e'{=}first(ctx(e)) \land e''{=}last(ctx(e)) ]$ \\ 
% Syncronization time& $sync(L',PN')=[|\pi_{ct}(e''){-}\pi_{ct}(e')| \mid pi \in PI_{L'} \land  e{=}first(pi) \land e'{=}first(en(e)) \land e''{=}en_{PN'}(e) ]$ \\ 
% \addlinespace
% \rowcolor[gray]{.9} 
% % Coherent Syncronization time & $[|\pi_{ct}(e''){-}\pi_{ct}(e')| \mid pi \in PI_{filt(L',S)} \land e{=}first(pi) \land |\pi_{omap}(e)(ot)| \ge 2 \land e'{=}first(ctx_{ot}(e)) \land e''{=}last(ctx_{ot}(e)) ]$ \\
% Coherent Syncronization time & $sync_{ot}(L',PN')=[|\pi_{ct}(e''){-}\pi_{ct}(e')| \mid pi \in PI_{L'} \land  e{=}first(pi) \land |\pi_{omap}(e)(ot)| \ge 2 \land e'{=}first(en(e,ot)) \land e''{=}last(en(e,ot)) ]$ \\
% \addlinespace
% Inherent Syncronization time & $[|\pi_{ct}(e''){-}\pi_{ct}(e')| \mid pi \in PI_{filt(L',S)} \land e{=}first(pi) \land |dom(\pi_{omap}(e))| \ge 2 \land ot,ot'\in dom(\pi_{omap}(e)) \land e'{=}last(ctx_{ot}(e)) \land e''{=}last(ctx_{ot'}(e)) ]$ \\
Syncronization time & $sync_{ot,ot'}(L',PN'){=}[|\pi_{ct}(e''){-}\pi_{ct}(e')| \mid pi \in PI_{L'} \land  e{=}first(pi) \land e'{=}en_{PN'}(e,ot) \land e''{=}en_{PN'}(e,ot') ]$ \\
\textbf{Non-temporal Metric} & \\
\rowcolor[gray]{.9} 
% Absolute Frequency  & $|PI_{OT',T'}|$ \\ 
Absolute Frequency  & $abs\_freq(L',PN'){=}|\{pi \in PI_{L'}\}|$ \\ 
% Unique Frequency    & $|\{id(pi) \mid pi \in PI_{filt(L',S)} \}|$ \\
% \addlinespace
Object Frequency    & $obj\_freq(L',PN')_{ot}{=}|\{oi \in \univ{oi} \mid (V,K) \in PI_{L'} \land e \in V \land oi \in \pi_{omap}(e)(ot) \}|$ \\
\rowcolor[gray]{.9} 
Object Type Frequency  & $obj\_type\_freq(L',PN'){=}|\{ot \in \univ{ot} \mid (V,K) \in PI_{L'} \land e \in V \land ot \in dom(\pi_{omap}(e)) \}|$ \\ 
Interacting Activity Frequency  & $int\_act\_freq(L',PN'){=}|\{\pi_{act}(e) \mid (V,K) \in PI_{L'} \land e \in V \land |dom(\pi_{omap}(e))| \ge 2 \}|$ \\ 
% Complete Frequency  & $thru(L_{S},ON_{S})=|pi \in PI_{filt(L',S)}|$ \\
% \addlinespace
% \rowcolor[gray]{.9} 
% Ongoing Frequency   & $thru(L_{S},ON_{S})=|ft_{ongoing}(PI_{filt(L',S)})|$ \\
% Queue& $|\{pi | cpi \in ft_{ongoing}(PI_{filt(L',S)}) \land e=last(pi) \land t \in enabled_{ON}(e)\}|$ \\
% \addlinespace
\bottomrule
\end{tabularx}
\label{tab:formal-derivation}
\end{table}

% \begin{table}
% \centering
% \caption{
% Let $L=(E,OT,O,\pi_{act}, \pi_{stime}, \pi_{ct}, \pi_{omap})$ be an object-centric event log.
% Let $\mathit{ON}{=}(N,\mathit{pt},F_{\mathit{var}})$ be an object-centric Petri net, where $N{=}(P,T,F,l)$.
% Let $S$ is a subprocess of $ON$.
% We assume that $L_{S}$ is perfectly fitting $ON_{S}$.
% % $ctx_{OT'}(e)=\bigcup_{ot \in OT'} ctx(e,ot)$
% }
% \smallskip
% \sisetup{table-format = 3.2}
% \begin{tabularx}{\textwidth}{lY}
% \toprule 
% \textbf{Performance Metric}  & \textbf{Formal Derivation} \\
% \midrule
% \textbf{Temporal Metric} & \\
% \addlinespace
% Throughput time     & $thru(L_{S},ON_{S})=[\pi_{ct}(e){-}\pi_{st}(e') \mid ceg \in CEG_{L_{S}} \land e{=}last(ceg) \land e'{=}first(ceg) ]$ \\
% \addlinespace
% \rowcolor[gray]{.9} 
% Sojourn time & $sojourn(L_{S},ON_{S})=[\pi_{ct}(e){-}\pi_{ct}(e') \mid ceg \in CEG_{L_{S}} \land e{=}last(ceg) \land e'{=}last(ctx_{OT'}(first(ceg)))]$ \\
% \addlinespace
% Waiting time& $wait(L_{S},ON_{S})=[\pi_{st}(e){-}\pi_{ct}(e') \mid ceg \in CEG_{L_{S}} \land e{=}first(ceg) \land e'{=}first(context_{OT'}(e)) ]$ \\ 
% \addlinespace
% \rowcolor[gray]{.9} 
% Coherent Syncronization time & $sync_{ot}(L_{S},ON_{S})=[\pi_{ct}(e''){-}\pi_{ct}(e') \mid ceg \in CEG_{L_{S}} \land e{=}first(ceg) \land |\pi_{omap}(e)(ot)| \ge 2 \land e'{=}first(ctx_{ot}(e)) \land e''{=}last(ctx_{ot}(e)) ]$ \\
% \addlinespace
% \rowcolor[gray]{.9} 
% Inherent Syncronization time & $sync(L_{S},ON_{S})=[\pi_{ct}(e''){-}\pi_{ct}(e') \mid ceg \in CEG_{L_{S}} \land e{=}first(ceg) \land e'{=}first(ctx_{OT'}(e)) \land e''{=}last(ctx_{OT'}(e)) ]$ \\
% \addlinespace
% Service time& $service(L_{S},ON_{S})=[\pi_{ct}(e){-}\pi_{st}(e') \mid ceg \in CEG_{L_{S}} \land e{=}last(ceg) \land e'{=}first(ceg) ]$ \\ 
% \textbf{Non-temporal Metric} & \\
% \addlinespace
% \rowcolor[gray]{.9} 
% Absolute Frequency  & $abs\_freq(L_{S},ON_{S})=|CEG_{OT',T'}|$ \\ 
% \addlinespace
% % Unique Frequency    & $|\{id(ceg) \mid ceg \in CEG_{L_{S}} \}|$ \\
% % \addlinespace
% \rowcolor[gray]{.9} 
% Object Frequency    & $obj\_freq_{ot}(L_{S},ON_{S})=|\{oi \mid (V,K,otmap) \in CEG_{OT',T'} \land e \in V \land oi \in \pi_{omap}(e) \land type(oi){=}ot \}|$ \\
% \addlinespace
% % Complete Frequency  & $thru(L_{S},ON_{S})=|ceg \in CEG_{L_{S}}|$ \\
% % \addlinespace
% % \rowcolor[gray]{.9} 
% % Ongoing Frequency   & $thru(L_{S},ON_{S})=|ft_{ongoing}(CEG_{OT',T'})|$ \\
% \addlinespace
% % Queue& $|\{pi | cpi \in ft_{ongoing}(CEG_{OT',T'}) \land e=last(pi) \land t \in enabled_{ON}(e)\}|$ \\
% % \addlinespace
% \bottomrule
% \end{tabularx}
% \label{tab:formal-derivation}
% \end{table}
